Static vs Dynamic SAGAs

SAGAs calculi (or simply SAGAs) have been proposed by Bruni et al. as a model for long-running transactions. The approach therein can be considered static, while a dynamic approach has been proposed by Lanese and Zavattaro. In this paper we first extend both static SAGAs (in the centralized interruption policy) and dynamic SAGAs to deal with nesting, then we compare the two approaches.

==> eptcsdata.tex <==
\providecommand{\firstpage}{51}
\providecommand{\publicationstatus}{Bliudze, Bruni, Grohmann, Silva (Eds.):\\Third Interaction and Concurrency Experience (ICE 2010)\\
EPTCS 38, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.38.7}{10.4204/EPTCS.38.7}}

